Real-Time Sampling-Based Safe Motion Planning for Robotic Manipulators in Dynamic Environments

In this paper, we present the main features of Dynamic Rapidly-exploring Generalized Bur Tree (DRGBT) algorithm, a sampling-based planner for dynamic environments. We provide a detailed time analysis and appropriate scheduling to facilitate a real-time operation. To this end, an extensive analysis is conducted to identify the time-critical routines and their dependence on the number of obstacles. Furthermore, information about the distance to obstacles is used to compute a structure called dynamic expanded bubble of free configuration space, which is then utilized to establish sufficient conditions for a guaranteed safe motion of the robot while satisfying all kinematic constraints. An extensive randomized simulation trial is conducted to compare the proposed algorithm to a competing state-of-the-art method. Finally, an experimental study on a real robot is carried out covering a variety of scenarios including those with human presence. The results show the effectiveness and feasibility of real-time execution of the proposed motion planning algorithm within a typical sensor-based arrangement, using cheap hardware and sequential architecture, without the necessity for GPUs or heavy parallelization.

==> Pseudocodes/DRGBT_v2.tex <==
\begin{algorithm}[h]
	\caption{DRGBMT* algorithm}
	\label{DRGBMT* algorithm pseudocode}
	\begin{algorithmic}[1]
		\Require $\bb{q}_{init},~ \bb{q}_{goal},~ \varepsilon,~ obstacles$
		\Ensure $goal\_reached,~ traversed\_path$
		
		\State $path \gets \mathtt{RGBMT^*}(\bb{q}_{init},~ \bb{q}_{goal})$ \Comment{SD}
		\State $traversed\_path \gets \bb{q}_{init}$ 
		\State $\bb{q}_{curr} \gets \bb{q}_{init}$ 
		\State $replanning \gets \False$ 
		
		\While{$\bb{q}_{curr}~ \neq ~\bb{q}_{goal}$} 
		\State $horizon \gets  \mathtt{generateHorizon}(\bb{q}_{curr},~ path)$ \Comment{$4\pm 2$}
		\State $status \gets advanced$ 
		
		\While{$status = advanced$} 
		\State $obstacles \gets \mathtt{updateObstacles}(obstacles)$ 
		\If{$\mathtt{checkCollision}(\bb{q}_{curr},~ obstacles)$} \Comment{SD}
		\State $goal\_reached \gets \False$ 
		\State \Return 
		\EndIf
		\State $d_c \gets \mathtt{computeDistance}(\bb{q}_{curr},~ obstacles)$ \Comment{SD}
		\State $horizon \gets \mathtt{updateHorizon}(horizon,~ d_c,~ path)$ \Comment{$10\pm 10$}
		\State $g\_bur \gets \mathtt{generateGBur}(\bb{q}_{curr},~ horizon,~ d_c,~ obstacles)$ \Comment{SD}
		\State $weights \gets \mathtt{computeNodeWeights}(g\_bur)$ \Comment{$0.5\pm 0.5$}
		\State $\bb{q}_{next} \gets \mathtt{getNextNode}(g\_bur,~ weights)$ 
		\State $[\bb{q}_{new},~ status] \gets \mathtt{interpolate}(\bb{q}_{curr}$, $\bb{q}_{next}$, $\varepsilon$) \Comment{$8\pm 11$}
		\If{$status = trapped$}
			\State $replanning \gets \True$
			\State $weights(\bb{q}_{next}) \gets 0$
		\Else
			\State $\bb{q}_{curr} \gets \bb{q}_{new}$
			\State $traversed\_path \gets [traversed\_path,~ \bb{q}_{curr}]$ 
		\EndIf
		
		\If{$replanning$ \Or $\mathtt{whetherToReplan}(weights)$} 
		\State $new\_path \gets \mathtt{RGBMT^*}$($\bb{q}_{curr}$, $\bb{q}_{goal}$) \Comment{SD}
		\If{$new\_path~\neq~ \emptyset$} 
			\State $path \gets \mathtt{updatePath}(new\_path$, $\bb{q}_{curr})$ 
			\State $replanning \gets \False$ 
			\State $status \gets reached$ 
		\Else
			\State $replanning \gets \True$ 
			\State $status \gets advanced$ 
		\EndIf
		\EndIf
		\EndWhile
		\EndWhile
		\State $goal\_reached \gets \True$ 
	\end{algorithmic}
\end{algorithm}
%\setlength{\textfloatsep}{0pt}% Remove \textfloatsep

==> Tables/tab_DRGBT_high_DoF_scenarios_results.tex <==
\begin{tabular}{c}
	\begin{tabular}{@{}lccc|ccc@{}}
	\cmidrule(l){2-7}
	& \multicolumn{3}{c|}{10-DoF robot} & \multicolumn{3}{c}{14-DoF robot} \\ 
	\cmidrule(l){2-7} 
	& DRGBT     & MARS & RRT$^\mathrm{X}$  & DRGBT     & MARS  & RRT$^\mathrm{X}$  \\ \midrule
	\multicolumn{1}{l|}{$\eta\,[\%]$}    
	& $\bb{89.1}$ ($\bb{7.3}$) & $68$ ($2.1$) & $44.6$ ($4.3$) & $\bb{65.1}$ ($\bb{31.6}$) & $58.4$ ($19.8$) & $34.7$ ($29.8$) \\
	\multicolumn{1}{l|}{$T_{alg}\,\mathrm{[s]}$} 
	& $\bb{8.6} \pm \bb{7.6}$ & $12.1\pm 7.4$ & $9.7\pm 4.9$ & $14.7\pm 13.0 $ & $17.6\pm 8.4$ & $\bb{11.3}\pm \bb{9.2}$ \\
	\multicolumn{1}{l|}{$D\,\mathrm{[rad]}$}   
	& $\bb{20.1}\pm \bb{14.4}$ & $23.0\pm 12.4$ & $21.2\pm 6.1$ & $37.8\pm 28.6$ & $33.7\pm 14.3$ & $\bb{26.1}\pm \bb{6.7}$ \\ \bottomrule
\end{tabular}
\\
\begin{tabular}{@{}lccc|ccc@{}}
	\cmidrule(l){2-7}
	& \multicolumn{3}{c|}{18-DoF robot} & \multicolumn{3}{c}{22-DoF robot} \\ 
	\cmidrule(l){2-7} 
	& DRGBT     & MARS & RRT$^\mathrm{X}$  & DRGBT     & MARS  & RRT$^\mathrm{X}$  \\ \midrule
	\multicolumn{1}{l|}{$\eta\,[\%]$}    
	& $\bb{41.2}$ ($\bb{57.1}$) & $37.5$ ($45.2$) & $29.4$ ($48$) & $\bb{23.5}$  ($\bb{73.6}$) & $3$ ($84.6$) & $22.4$ ($60.4$) \\
	\multicolumn{1}{l|}{$T_{alg}\,\mathrm{[s]}$} 
	& $16.9\pm 11.4$ & $20.6\pm 7.7$ & $\bb{10.1\pm 5.3}$ & $27\pm 17.5$ & $18.9\pm 8.3$ & $\bb{10\pm 3.7}$ \\
	\multicolumn{1}{l|}{$D\,\mathrm{[rad]}$}   
	& $48.3\pm 29.3$ & $41.9\pm 14.6$ & $\bb{30.2\pm 7.4}$ & $72.7\pm 44.3$ & $\bb{18.4\pm 6.2}$ & $33.4\pm 6.9$ \\ \bottomrule
\end{tabular}
\end{tabular}
